FP-Inconsistent: Measurement and Analysis of Fingerprint Inconsistencies in Evasive Bot Traffic

As browser fingerprinting is increasingly being used for bot detection, bots have started altering their fingerprints for evasion. We conduct the first large-scale evaluation of evasive bots to investigate whether and how altering fingerprints helps bots evade detection. To systematically investigate evasive bots, we deploy a honey site incorporating two anti-bot services (DataDome and BotD) and solicit bot traffic from 20 different bot services that purport to sell "realistic and undetectable traffic". Across half a million requests from 20 different bot services on our honey site, we find an average evasion rate of 52.93% against DataDome and 44.56% evasion rate against BotD. Our comparison of fingerprint attributes from bot services that evade each anti-bot service individually as well as bot services that evade both shows that bot services indeed alter different browser fingerprint attributes for evasion. Further, our analysis reveals the presence of inconsistent fingerprint attributes in evasive bots. Given evasive bots seem to have difficulty in ensuring consistency in their fingerprint attributes, we propose a data-driven approach to discover rules to detect such inconsistencies across space (two attributes in a given browser fingerprint) and time (a single attribute at two different points in time). These rules, which can be readily deployed by anti-bot services, reduce the evasion rate of evasive bots against DataDome and BotD by 48.11% and 44.95% respectively.

==> privacy_enhancing_tools.tex <==
\section{Privacy-enhancing technologies}
\label{sec:pet_eval}
Privacy-enhancing technologies such as Brave \cite{brave-browser},  Tor \cite{tor-browser}, and
Canvas Fingerprint Defender \cite{canvas-fingerprint-defender} alter browser attributes to protect 
the privacy of legitimate users from online trackers \cite{fp-inspector, oneclass-tracker-detection}.
\system to detect them as bots. In this section, we examine the browser attributes altered by such
technologies and measure their impact on \system. Our findings show that (1) the vast majority of 
privacy-enhancing technologies do not result in false positives with \system and (2) \botservs 
cannot abuse them for evasion since they alter a limited set of attributes.

\subsection{Analysis}
%In this section, we first describe our experimental methodology to analyze browser attributes among
%different privacy-enhancing technologies. We then present our results and analysis from running these
%experiments.
\subsubsection{Experimental Methodology}
We focus on three commonly used privacy-enhancing browsers, namely, Safari \cite{safari-browser}, 
Brave \cite{brave-browser} and Tor \cite{tor-browser} as well as two commonly used privacy-enhancing 
browser extensions, namely, uBlock Origin \cite{uBlock} and Adblock Plus \cite{AdblockPlus} on 
Google Chrome.

We first configured each privacy-enhancing tool to enable their strongest privacy protections and
sent requests from each tool to our honey site to capture their browser attributes. We sent a total of 300
requests from devices running macOS (M1 MacBook Pro), Linux (Intel Coffee Lake Desktop), iOS (iPad Pro), 
and Android (Google Pixel 7). We then evaluated \system against the captured browser attributes to
determine if they were detected as bots. Finally, we manually inspected the attributes to pinpoint the
alterations introduced by each technology.

\subsubsection{Results} 
\leavevmode\\
\textbf{uBlock Origin and AdBlock Plus} We report that none of the requests sent when using uBlock 
Origin and AdBlock Plus triggered any spatial or temporal inconsistencies. Inspecting the browser 
attributes from these requests showed that these extensions did not alter any browser attributes.
These extensions operate by detecting trackers and blocking them as opposed to altering browser 
attributes to protect privacy. These two extensions cater to over 80 million users combined
on the most widely used browser, Google Chrome \cite{browser_market, ublock_webstore, adblock_webstore}
showing that \system can detect bots while having zero impact of all these users.

\textbf{Safari} Safari does not alter browser attributes to protect privacy either, resulting in \system 
detecting none of the requests from Safari as emerging from bots. Safari has the second largest market
share among web browsers \cite{browser_market} showing that \system can detect bots without affecting
the large number of users who use Safari.

\textbf{Brave} We observe that Brave currently alters 6 different browser attributes:
\texttt{screenResolution}, \texttt{hardwareConcurrency}, \texttt{deviceMemory}, \texttt{audio}, 
\texttt{canvas}, and \texttt{plugins}. Of these, \system does not incorporate \texttt{audio}, 
\texttt{canvas}, and \texttt{plugins} as part of its detection rules. Brave's alterations to the other 
attributes did not trigger any spatial inconsistencies since they were consistent with the other
browser attributes. For instance, Brave alters \texttt{deviceMemory} on desktops to plausible values
(0.5, 1, 2, 4, and 8), which align with the amount of memory in typical desktops and remain consistent 
with other browser attributes.

However, since Brave does not automatically unset Cookies between requests, it triggered several temporal 
inconsistencies where multiple requests shared the same Cookie but had differing values for both 
\texttt{hardwareConcurrency} and \texttt{deviceMemory}. Such inconsistencies are rare in real-world scenarios, 
as they require users to enable Brave’s fingerprint protection while retaining Cookies. These rare false positives
can be mitigated using CAPTCHAs, with the verification result stored in Cookies (Section \ref{sec:fp_disc}).

Although \system does not detect requests from Brave as bots, we argue that \botservs cannot exploit Brave for 
evasion since they seek to alter attributes that are not supported by Brave.  Concretely, we see that Brave only 
alters 2 attributes that are most commonly altered by \smartbots (Section \ref{sec:measurement_attributes}) and
does not alter other attributes that are of interest to bots such as those pertaining to their device type or 
geolocation (Section \ref{sec:inconsistency_measurement}). If Brave were to alter more browser attributes 
in the future, \system could become prone to more false positives. However, even in such a hypothetical scenario, 
these false positives can be mitigated using CAPTCHAs (Section \ref{sec:fp_disc}. Moreover, only a small set of users would 
encounter these CAPTCHAs if Brave's market share continues to remain at 1\% \cite{brave-market-share}.

\textbf{Tor} \system detected all requests from Tor as bots since they triggered spatial inconsistencies between 
the geolocation inferred from their IP address and the \texttt{timezone} attribute of their navigator object.
While using Tor results in false positives, we expect them to affect a small set of users since Tor likely has 
less than 1\% market share \cite{browser_market}. Furthermore, most websites currently block requests from Tor 
\cite{tor-block}, due to the difficulty in distinguishing Tor traffic from bots. To mitigate false positives, 
we can present users with CAPTCHAs rather than blocking their requests (Section \ref{sec:fp_disc}).

\subsection{Coexistence of Bot Detection and Privacy-Enhancing Technologies} Overall, we observe that \system can 
detect bots without impeding most commonly used privacy-enhancing technologies (except Tor). This observation is 
interesting because many assume that the goals of bot detection and online tracking are identical. They believe 
that enhancements to bot detection would also bolster online tracking and weaken privacy-enhancing tools.

While bot detection and tracking overlap, tracking is a more complex problem as it seeks to uniquely identify each 
user. In contrast, bot detection solely seeks to determine if a particular request was generated by a bot. Accordingly,
altering any browser attribute enhances privacy by making it harder for trackers to link requests from the same user, 
even when other attributes remain unchanged. On the other hand, altering any browser attribute does not necessarily 
help bots with evasion since other attributes can still reveal their presence. This distinction between bot detection
and online tracking allows bot detection systems like \system to coexist with privacy-enhancing technologies.

==> tables/api_comparison_botd_datadome_fouanalytics.tex <==
\begin{table*}[]
    \centering
    \caption{Caption}
    \begin{tabular}{l c c c}
\toprule
                                      \textbf{Browser APIs} &   \textbf{DataDome} &       \textbf{BotD} & \textbf{FouAnalytics} \\
\midrule
        \multicolumn{4}{c}{\textbf{Display}} \\
        \midrule
                    window.screen.colorDepth & \tikzcmark & \tikzxmark &    \tikzcmark \\
                    HTMLCanvasElement.width & \tikzxmark & \tikzxmark &    \tikzcmark \\
                    HTMLCanvasElement.height & \tikzxmark & \tikzxmark &    \tikzcmark \\
                HTMLCanvasElement.getContext & \tikzcmark & \tikzcmark &    \tikzcmark \\
         CanvasRenderingContext2D.strokeText & \tikzxmark & \tikzxmark &    \tikzcmark \\

         \midrule
         \multicolumn{4}{c}{\textbf{Navigator}} \\
         \midrule
         
                  window.navigator.webdriver & \tikzcmark & \tikzcmark &    \tikzcmark \\
                  window.navigator.vendorSub & \tikzxmark & \tikzxmark &    \tikzcmark \\
                     window.navigator.vendor & \tikzcmark & \tikzcmark &    \tikzcmark \\
                  window.navigator.userAgent & \tikzcmark & \tikzcmark &    \tikzcmark \\
              window.navigator.serviceWorker & \tikzcmark & \tikzxmark &    \tikzxmark \\
                 window.navigator.sendBeacon & \tikzxmark & \tikzxmark &    \tikzcmark \\
                 window.navigator.productSub & \tikzxmark & \tikzcmark &    \tikzcmark \\
                    window.navigator.product & \tikzxmark & \tikzxmark &    \tikzcmark \\
                    window.navigator.plugins & \tikzcmark & \tikzcmark &    \tikzcmark \\
                   window.navigator.platform & \tikzcmark & \tikzxmark &    \tikzcmark \\
                window.navigator.permissions & \tikzcmark & \tikzcmark &    \tikzcmark \\
                      window.navigator.oscpu & \tikzcmark & \tikzxmark &    \tikzxmark \\
                  window.navigator.mimeTypes & \tikzcmark & \tikzcmark &    \tikzxmark \\
               window.navigator.mediaDevices & \tikzcmark & \tikzxmark &    \tikzcmark \\
             window.navigator.maxTouchPoints & \tikzcmark & \tikzxmark &    \tikzxmark \\
                  window.navigator.languages & \tikzcmark & \tikzcmark &    \tikzxmark \\
                   window.navigator.language & \tikzcmark & \tikzcmark &    \tikzcmark \\
        window.navigator.hardwareConcurrency & \tikzcmark & \tikzxmark &    \tikzcmark \\
                 window.navigator.doNotTrack & \tikzxmark & \tikzxmark &    \tikzcmark \\
              window.navigator.cookieEnabled & \tikzxmark & \tikzxmark &    \tikzcmark \\
                    window.navigator.buildID & \tikzcmark & \tikzxmark &    \tikzxmark \\
                 window.navigator.appVersion & \tikzxmark & \tikzcmark &    \tikzcmark \\
                    window.navigator.appName & \tikzxmark & \tikzxmark &    \tikzcmark \\
                window.navigator.appCodeName & \tikzxmark & \tikzxmark &    \tikzcmark \\
                  window.navigator.\_\_proto\_\_ & \tikzcmark & \tikzxmark &    \tikzxmark \\

            \midrule
         \multicolumn{4}{c}{\textbf{Storage}} \\
         \midrule
                      window.document.cookie & \tikzcmark & \tikzxmark &    \tikzxmark \\
                       window.sessionStorage & \tikzcmark & \tikzxmark &    \tikzcmark \\                            Storage.setItem & \tikzxmark & \tikzxmark &    \tikzcmark \\
                          Storage.removeItem & \tikzxmark & \tikzxmark &    \tikzcmark \\
                             Storage.getItem & \tikzxmark & \tikzxmark &    \tikzcmark \\
                                                     window.localStorage & \\tikzcmark & \\tikzxmark &    \\tikzcmark \\\\window.localStorage & \tikzcmark & \tikzxmark &    \tikzcmark \\

          \midrule
         \multicolumn{4}{c}{\textbf{Performance}} \\
         \midrule
                          Performance.timing & \tikzxmark & \tikzxmark &    \tikzcmark \\
                             Performance.now & \tikzcmark & \tikzxmark &    \tikzcmark \\
                      Performance.navigation & \tikzxmark & \tikzxmark &    \tikzcmark \\

        
          \midrule
         \multicolumn{4}{c}{\textbf{Audio}} \\
         \midrule
                         OscillatorNode.type & \tikzxmark & \tikzxmark &    \tikzcmark \\
                        OscillatorNode.start & \tikzxmark & \tikzxmark &    \tikzcmark \\
                    OscillatorNode.frequency & \tikzxmark & \tikzxmark &    \tikzcmark \\
                      OscillatorNode.connect & \tikzxmark & \tikzxmark &    \tikzcmark \\
          OfflineAudioContext.startRendering & \tikzxmark & \tikzxmark &    \tikzcmark \\
              OfflineAudioContext.oncomplete & \tikzxmark & \tikzxmark &    \tikzcmark \\
             OfflineAudioContext.destination & \tikzxmark & \tikzxmark &    \tikzcmark \\
        OfflineAudioContext.createOscillator & \tikzxmark & \tikzxmark &    \tikzcmark \\
OfflineAudioContext.createDynamicsCompressor & \tikzxmark & \tikzxmark &    \tikzcmark \\


          \midrule
         \multicolumn{4}{c}{\textbf{Mouse Movements}} \\
         \midrule
                             MouseEvent.type & \tikzcmark & \tikzxmark &    \tikzxmark \\
                        MouseEvent.timeStamp & \tikzcmark & \tikzxmark &    \tikzxmark \\
                           MouseEvent.target & \tikzxmark & \tikzxmark &    \tikzcmark \\
                            MouseEvent.pageY & \tikzxmark & \tikzxmark &    \tikzcmark \\
                            MouseEvent.pageX & \tikzxmark & \tikzxmark &    \tikzcmark \\
                          MouseEvent.clientY & \tikzcmark & \tikzxmark &    \tikzxmark \\
                          MouseEvent.clientX & \tikzcmark & \tikzxmark &    \tikzxmark \\
         %  \midrule
         % \multicolumn{4}{c}{\textbf{Miscellaneous}} \\
         % \midrule

         %            window.document.referrer & \tikzxmark & \tikzxmark &    \tikzcmark \\
         %             window.addEventListener & \tikzcmark & \tikzxmark &    \tikzcmark \\
\bottomrule
\end{tabular}
    \label{tab:my_label}
\end{table*}

==> tables/botd_adv.tex <==
\begin{table}[t]
\centering
  \caption{\botd 's detection rate on 1000 browser fingerprints with attributes that were detected in the wild, their randomly perturbed counterparts and adversarially perturbed counterparts.}
  \label{tab:botd_adv}
\begin{tabular}{c c}
  \hline
  \textbf{Perturbation type} & \textbf{Detection Rate}\\
  \hline
  No perturbation & 100\%\\

  Random perturbation & 96.9\%\\

  Adversarial perturbation & 0\%\\
  \hline
\end{tabular}
\end{table}

==> tables/botd_tp_fn.tex <==
\begin{table*}[t]
  \centering
  \small
  \begin{tabular}{|l|c|c|c|}
    \hline
    {\bf{Service}} & {\bf{Number of}} & {\bf{BotD}}           & {\bf{BotD}}            \\
    {\bf{Name}}    & {\bf{requests}}  & {\bf{True Positives}} & {\bf{False Negatives}} \\ \hline
    {gSiqhkdp71}   & {16796}          & {27.46}               & {72.54}                \\ \hline
    {Byxxodkxn3}   & {30832}          & {27.56}               & {72.44}                \\ \hline
    {1UHvZJM5nd}   & {13586}          & {76.69}               & {23.31}                \\ \hline
    {Ofauw8YynZ}   & {6080}           & {39.79}               & {60.21}                \\ \hline
    {gL7oFe6cYy}   & {2667}           & {10.65}               & {89.35}                \\ \hline
    {pqHlMpbwth}   & {2949}           & {42.42}               & {57.58}                \\ \hline
    {qx9V0qaFGF}   & {4207}           & {100.0}               & {0.0}                  \\ \hline
    {qkfN2dVsSP}   & {4461}           & {64.45}               & {35.55}                \\ \hline
    {3JlDf2IKe2}   & {839}            & {0.0}                 & {100.0}                \\ \hline
    {D9ixPIU9HT}   & {974}            & {100.0}               & {0.0}                  \\ \hline
    {cbWdBCf38N}   & {3135}           & {41.21}               & {58.79}                \\ \hline
    {7jlJc1as8L}   & {2225}           & {99.96}               & {0.04}                 \\ \hline
    {J1Akzg6fRB}   & {3312}           & {67.6}                & {32.4}                 \\ \hline
    {HwFp9ABpSW}   & {1009}           & {0.0}                 & {100.0}                \\ \hline
  \end{tabular}
  \caption{Caption}
  \label{fig:botd_decisions}
\end{table*}


==> tables/datadome_tp_fn.tex <==
\begin{table*}[t]
  \centering
  \small
  \begin{tabular}{|l|c|c|c|}
    \hline
    {\bf{Service}} & {\bf{Number of}} & {\bf{DataDome}}       & {\bf{DataDome}}        \\
    {\bf{Name}}    & {\bf{requests}}  & {\bf{True Positives}} & {\bf{False Negatives}} \\ \hline
    {gSiqhkdp71}   & {16796}          & {58.45}               & {41.55}                \\ \hline
    {Byxxodkxn3}   & {30832}          & {55.29}               & {44.71}                \\ \hline
    {1UHvZJM5nd}   & {13586}          & {20.55}               & {79.45}                \\ \hline
    {Ofauw8YynZ}   & {6080}           & {92.62}               & {7.38}                 \\ \hline
    {gL7oFe6cYy}   & {2667}           & {19.46}               & {80.54}                \\ \hline
    {pqHlMpbwth}   & {2949}           & {91.18}               & {8.82}                 \\ \hline
    {qx9V0qaFGF}   & {4207}           & {98.19}               & {1.81}                 \\ \hline
    {qkfN2dVsSP}   & {4461}           & {20.35}               & {79.65}                \\ \hline
    {3JlDf2IKe2}   & {839}            & {89.27}               & {10.73}                \\ \hline
    {D9ixPIU9HT}   & {974}            & {98.87}               & {1.13}                 \\ \hline
    {cbWdBCf38N}   & {3135}           & {82.33}               & {17.67}                \\ \hline
    {7jlJc1as8L}   & {2225}           & {96.94}               & {3.06}                 \\ \hline
    {J1Akzg6fRB}   & {3312}           & {19.2}                & {80.8}                 \\ \hline
    {HwFp9ABpSW}   & {1009}           & {86.82}               & {13.18}                \\ \hline
  \end{tabular}
  \caption{Caption}
  \label{fig:datadome_decisions}
\end{table*}

==> tables/inconsistency_analysis_direct.tex <==
\begin{table*}[ht]
\centering
\caption{Direct Inconsistency Examples}
\begin{tabular}{l|c|c|l}
\toprule
\textbf{Feature Group} & \textbf{Feature Pair} & \textbf{Example} \\
\midrule
\multirow{5}{*}{Location} & \multirow{5}{*}{(IP Location, Time Zone)} & \texttt{(France/Hauts-de-France, America/Los Angeles)} \\[0.5ex]
 &  & \texttt{(Germany/Sachsen, America/Los Angeles)} \\[0.5ex]
 &  & \texttt{(Singapore/Singapore, America/Los Angeles)} \\[0.5ex]
 &  & \texttt{(United States of America/California, Asia/Shanghai)} \\[0.5ex]
 &  & \texttt{(United States of America/Virginia, Pacific/Auckland)} \\[0.5ex]
\bottomrule
\end{tabular}
\label{table:direct_inconsistencies}
\end{table*}

==> tables/kl_botd_cont.tex <==
\begin{table}[h]
\centering
  \caption{Continuous attributes which differ the most among requests which were detected and evaded BotD}
  \label{tab:kl_botd_cont}
\begin{tabular}{ c c }
  \hline
  \textbf{Attribute} & \textbf{KL Divergence}\\
  \hline
  Width of Sans-serif font & 0.47\\
  
  Width of minimum font & 0.45\\
  
  Maximum number of touch points & 0.24\\
  
  Number of CPU cores & 0.11\\
  
  Amount of memory & 0.16\\
  \hline
\end{tabular}
\end{table}

==> tables/kl_dd_cont.tex <==
\begin{table}[h]
\centering
  \caption{Continuous attributes which differ the most among requests which were detected and evaded DataDome}
  \label{tab:kl_dd_cont}
\begin{tabular}{ c c }
  \hline
  \textbf{Attribute} & \textbf{KL Divergence} \\
  \hline
  Width of Monospace font & 0.23 \\
  
  Number of CPU cores & 0.18 \\
  
  Maximum number of touch points & 0.11\\
  
  Width of Sans-serif font & 0.11 \\
  
  Amount of memory & 0.08 \\
  \hline
\end{tabular}
\end{table}

==> tables/service_decisions.tex <==
\begin{table*}[t]
	\centering
	\small
	\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
		%\begin{tabular}{@{}ll@{}}
		\hline
		{\bf{Service}} & \multicolumn{4}{|c|}{\bf{Num. Reqs}} & \multicolumn{4}{|c|}{\bf{Num. IPs}} & \multicolumn{4}{|c|}{\bf{Num. fingerprints}} & \multicolumn{4}{|c|}{\bf{Num.cookies}}                                                                                                                                                                                                                                               \\
		{}             & \multicolumn{2}{|c}{\bf{Datadome}}   & \multicolumn{2}{|c|}{\bf{BotD}}     & \multicolumn{2}{|c}{\bf{Datadome}}           & \multicolumn{2}{|c|}{\bf{BotD}}        & \multicolumn{2}{|c}{\bf{Datadome}} & \multicolumn{2}{|c|}{\bf{BotD}} & \multicolumn{2}{|c}{\bf{Datadome}} & \multicolumn{2}{|c|}{\bf{BotD}}                                                                                                 \\
		{}             & {\bf{TP}}                            & {\bf{FN}}                           & {\bf{TP}}                                    & {\bf{FN}}                              & {\bf{TP}}                          & {\bf{FN}}                       & {\bf{TP}}                          & {\bf{FN}}                       & {\bf{TP}} & {\bf{FN}} & {\bf{TP}} & {\bf{FN}} & {\bf{TP}} & {\bf{FN}} & {\bf{TP}} & {\bf{FN}} \\ \hline
		{gSiqhkdp71}   & {4612}                               & {12184}                             & {9817}                                       & {6979}                                 & {1238}                             & {2536}                          & {1981}                             & {1953}                          & {1810}    & {4974}    & {4055}    & {2970}    & {1778}    & {4909}    & {3994}    & {2934}    \\ \hline
		{Byxxodkxn3}   & {8498}                               & {22334}                             & {17047}                                      & {13785}                                & {2805}                             & {4284}                          & {3662}                             & {3628}                          & {5284}    & {14416}   & {10965}   & {9003}    & {5239}    & {14281}   & {10849}   & {8933}    \\ \hline
		{1UHvZJM5nd}   & {10419}                              & {3167}                              & {2792}                                       & {10794}                                & {4502}                             & {2109}                          & {1338}                             & {4558}                          & {3324}    & {1454}    & {1295}    & {3880}    & {10260}   & {3033}    & {2658}    & {10203}   \\ \hline
		{Ofauw8YynZ}   & {2419}                               & {3661}                              & {5631}                                       & {449}                                  & {358}                              & {374}                           & {382}                              & {207}                           & {831}     & {474}     & {1212}    & {287}     & {1805}    & {2744}    & {4235}    & {417}     \\ \hline
		{gL7oFe6cYy}   & {284}                                & {2383}                              & {519}                                        & {2148}                                 & {267}                              & {1614}                          & {410}                              & {1469}                          & {210}     & {1870}    & {465}     & {1672}    & {280}     & {2154}    & {482}     & {1933}    \\ \hline
		{pqHlMpbwth}   & {1251}                               & {1698}                              & {2689}                                       & {260}                                  & {242}                              & {253}                           & {261}                              & {130}                           & {530}     & {280}     & {747}     & {188}     & {932}     & {1280}    & {2032}    & {240}     \\ \hline
		{qx9V0qaFGF}   & {4207}                               & {0}                                 & {4131}                                       & {76}                                   & {179}                              & {0}                             & {176}                              & {39}                            & {111}     & {0}       & {109}     & {30}      & {2068}    & {0}       & {2033}    & {50}      \\ \hline
		{qkfN2dVsSP}   & {2875}                               & {1586}                              & {908}                                        & {3553}                                 & {1795}                             & {1129}                          & {612}                              & {2055}                          & {1245}    & {1043}    & {606}     & {1838}    & {2845}    & {1508}    & {875}     & {3379}    \\ \hline
		{3JlDf2IKe2}   & {0}                                  & {839}                               & {749}                                        & {90}                                   & {0}                                & {50}                            & {43}                               & {9}                             & {0}       & {62}      & {55}      & {8}       & {0}       & {55}      & {48}      & {9}       \\ \hline
		{D9ixPIU9HT}   & {974}                                & {0}                                 & {963}                                        & {11}                                   & {108}                              & {0}                             & {108}                              & {7}                             & {68}      & {0}       & {68}      & {5}       & {595}     & {0}       & {590}     & {8}       \\ \hline
		{cbWdBCf38N}   & {1292}                               & {1843}                              & {2581}                                       & {554}                                  & {221}                              & {253}                           & {269}                              & {184}                           & {622}     & {471}     & {886}     & {348}     & {1001}    & {1448}    & {2053}    & {537}     \\ \hline
		{7jlJc1as8L}   & {2224}                               & {1}                                 & {2157}                                       & {68}                                   & {178}                              & {1}                             & {172}                              & {38}                            & {107}     & {1}       & {105}     & {31}      & {1284}    & {1}       & {1249}    & {44}      \\ \hline
		{J1Akzg6fRB}   & {2239}                               & {1073}                              & {636}                                        & {2676}                                 & {1160}                             & {679}                           & {361}                              & {1240}                          & {702}     & {468}     & {344}     & {964}     & {2210}    & {988}     & {575}     & {2422}    \\ \hline
		{HwFp9ABpSW}   & {0}                                  & {1009}                              & {876}                                        & {133}                                  & {0}                                & {105}                           & {90}                               & {27}                            & {0}       & {71}      & {60}      & {21}      & {0}       & {136}     & {123}     & {27}      \\ \hline
	\end{tabular}
	\caption{Caption}
	\label{fig:detection_stats}
\end{table*}

==> tables/service_decisions_fp_fn.tex <==
\begin{table*}[t]
	\centering
	\small
	\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
		%\begin{tabular}{@{}ll@{}}
		\hline
		{\bf{Service}} & \multicolumn{4}{|c|}{\bf{Num. Reqs}} & \multicolumn{4}{|c|}{\bf{Num. IPs}} & \multicolumn{4}{|c|}{\bf{Num. fingerprints}} & \multicolumn{4}{|c|}{\bf{Num.cookies}}                                                                                                                                                                                                                                               \\
		{}             & \multicolumn{2}{|c}{\bf{Datadome}}   & \multicolumn{2}{|c|}{\bf{BotD}}     & \multicolumn{2}{|c}{\bf{Datadome}}           & \multicolumn{2}{|c|}{\bf{BotD}}        & \multicolumn{2}{|c}{\bf{Datadome}} & \multicolumn{2}{|c|}{\bf{BotD}} & \multicolumn{2}{|c}{\bf{Datadome}} & \multicolumn{2}{|c|}{\bf{BotD}}                                                                                                 \\
		{}             & {\bf{TP}}                            & {\bf{FN}}                           & {\bf{TP}}                                    & {\bf{FN}}                              & {\bf{TP}}                          & {\bf{FN}}                       & {\bf{TP}}                          & {\bf{FN}}                       & {\bf{TP}} & {\bf{FN}} & {\bf{TP}} & {\bf{FN}} & {\bf{TP}} & {\bf{FN}} & {\bf{TP}} & {\bf{FN}} \\ \hline
		{gSiqhkdp71}   & {4612}                               & {12184}                             & {9817}                                       & {6979}                                 & {1238}                             & {2536}                          & {1981}                             & {1953}                          & {1810}    & {4974}    & {4055}    & {2970}    & {1778}    & {4909}    & {3994}    & {2934}    \\ \hline
		{Byxxodkxn3}   & {8498}                               & {22334}                             & {17047}                                      & {13785}                                & {2805}                             & {4284}                          & {3662}                             & {3628}                          & {5284}    & {14416}   & {10965}   & {9003}    & {5239}    & {14281}   & {10849}   & {8933}    \\ \hline
		{1UHvZJM5nd}   & {10419}                              & {3167}                              & {2792}                                       & {10794}                                & {4502}                             & {2109}                          & {1338}                             & {4558}                          & {3324}    & {1454}    & {1295}    & {3880}    & {10260}   & {3033}    & {2658}    & {10203}   \\ \hline
		{Ofauw8YynZ}   & {2419}                               & {3661}                              & {5631}                                       & {449}                                  & {358}                              & {374}                           & {382}                              & {207}                           & {831}     & {474}     & {1212}    & {287}     & {1805}    & {2744}    & {4235}    & {417}     \\ \hline
		{gL7oFe6cYy}   & {284}                                & {2383}                              & {519}                                        & {2148}                                 & {267}                              & {1614}                          & {410}                              & {1469}                          & {210}     & {1870}    & {465}     & {1672}    & {280}     & {2154}    & {482}     & {1933}    \\ \hline
		{pqHlMpbwth}   & {1251}                               & {1698}                              & {2689}                                       & {260}                                  & {242}                              & {253}                           & {261}                              & {130}                           & {530}     & {280}     & {747}     & {188}     & {932}     & {1280}    & {2032}    & {240}     \\ \hline
		{qx9V0qaFGF}   & {4207}                               & {0}                                 & {4131}                                       & {76}                                   & {179}                              & {0}                             & {176}                              & {39}                            & {111}     & {0}       & {109}     & {30}      & {2068}    & {0}       & {2033}    & {50}      \\ \hline
		{qkfN2dVsSP}   & {2875}                               & {1586}                              & {908}                                        & {3553}                                 & {1795}                             & {1129}                          & {612}                              & {2055}                          & {1245}    & {1043}    & {606}     & {1838}    & {2845}    & {1508}    & {875}     & {3379}    \\ \hline
		{3JlDf2IKe2}   & {0}                                  & {839}                               & {749}                                        & {90}                                   & {0}                                & {50}                            & {43}                               & {9}                             & {0}       & {62}      & {55}      & {8}       & {0}       & {55}      & {48}      & {9}       \\ \hline
		{D9ixPIU9HT}   & {974}                                & {0}                                 & {963}                                        & {11}                                   & {108}                              & {0}                             & {108}                              & {7}                             & {68}      & {0}       & {68}      & {5}       & {595}     & {0}       & {590}     & {8}       \\ \hline
		{cbWdBCf38N}   & {1292}                               & {1843}                              & {2581}                                       & {554}                                  & {221}                              & {253}                           & {269}                              & {184}                           & {622}     & {471}     & {886}     & {348}     & {1001}    & {1448}    & {2053}    & {537}     \\ \hline
		{7jlJc1as8L}   & {2224}                               & {1}                                 & {2157}                                       & {68}                                   & {178}                              & {1}                             & {172}                              & {38}                            & {107}     & {1}       & {105}     & {31}      & {1284}    & {1}       & {1249}    & {44}      \\ \hline
		{J1Akzg6fRB}   & {2239}                               & {1073}                              & {636}                                        & {2676}                                 & {1160}                             & {679}                           & {361}                              & {1240}                          & {702}     & {468}     & {344}     & {964}     & {2210}    & {988}     & {575}     & {2422}    \\ \hline
		{HwFp9ABpSW}   & {0}                                  & {1009}                              & {876}                                        & {133}                                  & {0}                                & {105}                           & {90}                               & {27}                            & {0}       & {71}      & {60}      & {21}      & {0}       & {136}     & {123}     & {27}      \\ \hline
	\end{tabular}
	\caption{Caption}
	\label{fig:detection_stats}
\end{table*}

==> tables/services_intersection_tp_fn.tex <==
\begin{table*}[t]
	\centering
	\small
	\begin{tabular}{|l|c|c|c|}
		\hline
		{\bf{Service}} & {\bf{Number of}} & {\bf{Intersection}}   & {\bf{Intersection}}    \\
		{\bf{Name}}    & {\bf{requests}}  & {\bf{True Positives}} & {\bf{False Negatives}} \\ \hline
		{gSiqhkdp71}   & {16796}          & {18.34}               & {81.66}                \\ \hline
		{Byxxodkxn3}   & {30832}          & {17.47}               & {82.53}                \\ \hline
		{1UHvZJM5nd}   & {13586}          & {15.56}               & {84.44}                \\ \hline
		{Ofauw8YynZ}   & {6080}           & {33.77}               & {66.23}                \\ \hline
		{gL7oFe6cYy}   & {2667}           & {1.95}                & {98.05}                \\ \hline
		{pqHlMpbwth}   & {2949}           & {34.99}               & {65.01}                \\ \hline
		{qx9V0qaFGF}   & {4207}           & {98.19}               & {1.81}                 \\ \hline
		{qkfN2dVsSP}   & {4461}           & {12.69}               & {87.31}                \\ \hline
		{3JlDf2IKe2}   & {839}            & {0.0}                 & {100.0}                \\ \hline
		{D9ixPIU9HT}   & {974}            & {98.87}               & {1.13}                 \\ \hline
		{cbWdBCf38N}   & {3135}           & {24.98}               & {75.02}                \\ \hline
		{7jlJc1as8L}   & {2225}           & {96.94}               & {3.06}                 \\ \hline
		{J1Akzg6fRB}   & {3312}           & {12.35}               & {87.65}                \\ \hline
		{HwFp9ABpSW}   & {1009}           & {0.0}                 & {100.0}                \\ \hline
	\end{tabular}
	\caption{Caption}
	\label{fig:intersection_decisions}
\end{table*}

==> tables/services_union_tp_fn.tex <==

\begin{table*}[t]
	\centering
	\small
	\begin{tabular}{|l|c|c|c|}
		\hline
		{\bf{Service}} & {\bf{Number of}} & {\bf{Union}}          & {\bf{Union}}           \\
		{\bf{Name}}    & {\bf{requests}}  & {\bf{True Positives}} & {\bf{False Negatives}} \\ \hline
		{gSiqhkdp71}   & {16796}          & {67.56}               & {32.44}                \\ \hline
		{Byxxodkxn3}   & {30832}          & {65.38}               & {34.62}                \\ \hline
		{1UHvZJM5nd}   & {13586}          & {81.68}               & {18.32}                \\ \hline
		{Ofauw8YynZ}   & {6080}           & {98.63}               & {1.37}                 \\ \hline
		{gL7oFe6cYy}   & {2667}           & {28.16}               & {71.84}                \\ \hline
		{pqHlMpbwth}   & {2949}           & {98.61}               & {1.39}                 \\ \hline
		{qx9V0qaFGF}   & {4207}           & {100.0}               & {0.0}                  \\ \hline
		{qkfN2dVsSP}   & {4461}           & {72.11}               & {27.89}                \\ \hline
		{3JlDf2IKe2}   & {839}            & {89.27}               & {10.73}                \\ \hline
		{D9ixPIU9HT}   & {974}            & {100.0}               & {0.0}                  \\ \hline
		{cbWdBCf38N}   & {3135}           & {98.56}               & {1.44}                 \\ \hline
		{7jlJc1as8L}   & {2225}           & {99.96}               & {0.04}                 \\ \hline
		{J1Akzg6fRB}   & {3312}           & {74.46}               & {25.54}                \\ \hline
		{HwFp9ABpSW}   & {1009}           & {86.82}               & {13.18}                \\ \hline
	\end{tabular}
	\caption{Caption}
	\label{fig:union_decisions}
\end{table*}
